Improving Rogers' upper bound for the density of unit ball packings via estimating the surface area of Voronoi cells from below in Euclidean d-space for all d>7

The sphere packing problem asks for the densest packing of unit balls in d-dimensional Euclidean space. This problem has its roots in geometry, number theory and it is part of Hilbert's 18th problem. In 1958 C. A. Rogers proved a non-trivial upper bound for the density of unit ball packings in d-dimensional Euclidean space for all d>0. In 1978 Kabatjanskii and Levenstein improved this bound for large d. In fact, Rogers' bound is the presently known best bound for 43>d>3, and above that the Kabatjanskii-Levenstein bound takes over. In this paper we improve Rogers' upper bound for the density of unit ball packings in Euclidean d-space for all d>7. We do this by estimating from below the surface area of Voronoi cells in any packing of unit balls in Euclidean d-space for all d>7.

==> FIG.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  FIG.tex
%		--- including ps figures in TeX documents
%
%               Maorong Zou, Feb. 24, 1993. Modified from 
%               Trevor J. Darrell's psfig.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       
%            !!!  USE AT YOUR OWN RISK !!!
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Description:
% 
%           Under dvi2ps, this set of macros is capable of
%    including up to four postscript figures a time. Figures
%    will be automatically positioned, provided that you supply
%    them some minimal information about your figures.
%
%
%  Usage: (see explaination below)
%
%     \OneFigure{file=FILE,llx=LLX,lly=LLY,urx=URX,ury=URY,
%		 width=WIDTH,height=HEIGHT}{caption}
%
%     \TwoFigures{filea=FILEA,llxa=LLXA, ... }
%		   {fileb=FILEB,llxb=LLXB, ...} {captioon}
%
%     \ThreeFigures{filea=...}{fileb=...}{filec=...}{caption}
%
%     \ThreeFiguresAB{ }   % same as \ThreeFigures{ }
%
%     \ThreeFiguresBA{ }   % same as \ThreeFigures{ }
%
%     \FourFigures{filea=FILEA, ...}{fileb=FILEB, ...}
%                 {filec=FILEC, ...}{filed=FILED, ...} {caption}
%
% !!! There must be no spaces inside any arguments (except caption),
% !!! each argument can be at most one line long.
%------------------------------------------------------------------
% Remarks:
%  
% 1. If your psfile has a line
%   	 %%BoundingBox # # # # 
%    and you want to use them as the bounding box for your
%    figure. leave `llx', `lly', `urx' and `ury' undefined.
%    These macros will search your ps file for BoundingBox.
%
% 2. If you want the aspect ratio of your figure be
%    preserved, leave one of `width?' and `height?'
%    undefined. (the other one will be automactically
%    computed according to the aspect ratio)
%
% 3.  In \TwoFigures ... \FourFigures, you can define the length
%     of the horizontal space between two adjacent figures by adding
%     an description      hsep=HSEP  in the first argument.
%     Similarly, you can control the vertical space between the
%     two vertically stacked figures in \ThreeFiguresAB(BA) by 
%     adding an description  vsep=VSEP. 
%
%------------------------------------------------------------------ 
%  Meaning of arguments:
%
%   FILE:        name of the postscript file
%   (LLX,LLY):   lower-left corner of the original picture, in points    
%   (URX,URY):   upper-right corner of the original picture, in points
%                (LLX LLY URX URY is the bounding box for your figure.)
% 
%   WIDTH:       width of the figure in your TeX doc, in pts
%   HEIGHT:      height of the figure in your TeX doc, in points
%   CAPTION:     caption: at most one line long
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=11\relax
\newwrite\@unused
\def\typeout#1{{\let\protect\string\immediate\write\@unused{#1}}}
\typeout{----- FIG.tex, version 1.0, April 27, 1993}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Arithmetic
%
\def\in@max#1#2#3{		 % result = max(#1, #2, #3) 
	\count201=#1
	\count202=#2
	\count203=#3
	\ifnum \count201 > \count202
		\edef\@maxa{\number\count201}
	\else
		\edef\@maxa{\number\count202}
	\fi
	\ifnum \@maxa > \count203
		\edef\@result{\number\@maxa}
	\else
		\edef\@result{\number\count203}
	\fi
}

\def\in@difference#1#2{		 % result =  #1 - #2 
	\count204 = #1
	\count205 = #2
	\advance \count204 by -\count205
	\edef\@result{\number\count204}
}

\def\in@sum#1#2{ 		% result = #1 + #2
	\count206 = #1
	\count207 = #2
	\advance \count206 by \count207
	\edef\@result{\number\count206}
}

\def\in@times#1#2{  		% result = #1 * #2
	\count208 =#1
	\count209 =#2
	\multiply \count208 by \count209
	\edef\@result{\number\count208}
}

\def\in@quotient#1#2{		% quotient = [ #1/#2], 
                      		% reminder =10 ( #1 - #2 quotient)
	\count210= #1
	\count211= #2
	\count212= #1
	\divide \count210 by \count211
	\edef\@quotient{\number\count210}
	\multiply \count210 by \count211
	\advance \count212 by -\count210
	\multiply \count212 by 10
	\edef\@reminder{\number\count212}
}

\def\in@atbdc#1#2#3{          % result = int ( #1 * #2/#3)
	\in@times{#1}{#2} \edef\@prod{\number\@result}
	\in@quotient{\@prod}{#3} \edef\@result{\number\@quotient}
}
\def\in@compdim#1#2#3#4#5{    % result = #5 (#2 -#1)/(#4 - #3)
	\in@difference{#2}{#1} \edef\@numera{\number\@result}
	\in@difference{#4}{#3} \edef\@denomi{\number\@result}
	\in@atbdc{#5}{\@numera}{\@denomi} 
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   loop structure (same as LaTeX `for'). used to parse args.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\@nnil{\@nil}
\def\@empty{}
\def\@psdonoop#1\@@#2#3{}
\def\@psdo#1:=#2\do#3{\edef\@psdotmp{#2}\ifx\@psdotmp\@empty \else
    \expandafter\@psdoloop#2,\@nil,\@nil\@@#1{#3}\fi}
\def\@psdoloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\@nnil \else
       #5\def#4{#2}\ifx #4\@nnil \else#5\@ipsdoloop #3\@@#4{#5}\fi\fi}
\def\@ipsdoloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\@nnil 
       \let\@nextwhile=\@psdonoop \else
      #4\relax\let\@nextwhile=\@ipsdoloop\fi\@nextwhile#2\@@#3{#4}}
\def\@tpsdo#1:=#2\do#3{\xdef\@psdotmp{#2}\ifx\@psdotmp\@empty \else
    \@tpsdoloop#2\@nil\@nil\@@#1{#3}\fi}
\def\@tpsdoloop#1#2\@@#3#4{\def#3{#1}\ifx #3\@nnil 
       \let\@nextwhile=\@psdonoop \else
      #4\relax\let\@nextwhile=\@tpsdoloop\fi\@nextwhile#2\@@#3{#4}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\def\@setparms#1=#2,{\@cs@name{@p@@s#1}{#2}}
\def\@cs@name#1{\csname #1\endcsname}
\def\parse@ps@parms#1{
	 	\@psdo\@rargs:=#1\do
		   {\expandafter\@setparms\@rargs,}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Flags
%
\newif\if@llx \newif\if@lly \newif\if@urx \newif\if@ury
\newif\if@height \newif\if@width \newif\if@pfile
%
\newif\if@llxa \newif\if@llya \newif\if@urxa \newif\if@urya 
\newif\if@heighta \newif\if@widtha \newif\if@pfilea  
%
\newif\if@llxb \newif\if@llyb \newif\if@urxb \newif\if@uryb
\newif\if@heightb \newif\if@widthb \newif\if@pfileb 
%
\newif\if@llxc \newif\if@llyc \newif\if@urxc \newif\if@uryc
\newif\if@heightc \newif\if@widthc \newif\if@pfilec
%
\newif\if@twofig \newif\if@threefig \newif\if@threefigab
\newif\if@threefigba \newif\if@fourfig
%
\newif\if@wh \newif\if@wha \newif\if@whb \newif\if@whc
%
\newif\if@hsepd \newif\if@vsepd 
%
\newif\if@nobbwarn \newif\if@nowhwarn 
\@nobbwarnfalse \@nowhwarnfalse
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 	Parsing argments
%
\def\@p@@sllx#1{\@llxtrue \count157=#1 \edef\@p@sllx{\number\count157}}
\def\@p@@sllxd#1{\@llxtrue \count157=#1 \edef\@p@sllx{\number\count157}}
\def\@p@@slly#1{\@llytrue \count157=#1 \edef\@p@slly{\number\count157}}
\def\@p@@sllyd#1{\@llytrue \count157=#1	\edef\@p@slly{\number\count157}}
\def\@p@@surx#1{\@urxtrue \count157=#1 \edef\@p@surx{\number\count157}}
\def\@p@@surxd#1{\@urxtrue \count157=#1 \edef\@p@surx{\number\count157}}
\def\@p@@sury#1{\@urytrue \count157=#1 \edef\@p@sury{\number\count157}}
\def\@p@@suryd#1{\@urytrue \count157=#1 \edef\@p@sury{\number\count157}}
\def\@p@@sheight#1{\@heighttrue \@whtrue \count157=#1
	   		\edef\@p@sheight{\number\count157}}
\def\@p@@sheightd#1{\@heighttrue \@whtrue\count157=#1
	   		\edef\@p@sheight{\number\count157}}
\def\@p@@swidth#1{\@widthtrue \@whtrue \count157=#1
			\edef\@p@swidth{\number\count157}}
\def\@p@@swidthd#1{\@widthtrue \@whtrue	\count157=#1
			\edef\@p@swidth{\number\count157}}

\def\@p@@sllxa#1{\@llxatrue \count157=#1 \edef\@p@sllxa{\number\count157}}
\def\@p@@sllya#1{\@llyatrue \count157=#1 \edef\@p@sllya{\number\count157}}
\def\@p@@surxa#1{\@urxatrue \count157=#1 \edef\@p@surxa{\number\count157}}
\def\@p@@surya#1{\@uryatrue \count157=#1 \edef\@p@surya{\number\count157}}
\def\@p@@sheighta#1{\@heightatrue \@whatrue \count157=#1
			\edef\@p@sheighta{\number\count157}}
\def\@p@@swidtha#1{\@widthatrue \@whatrue \count157=#1
			\edef\@p@swidtha{\number\count157}}
\def\@p@@sllxb#1{\@llxbtrue \count157=#1 \edef\@p@sllxb{\number\count157}}
\def\@p@@sllyb#1{\@llybtrue \count157=#1 \edef\@p@sllyb{\number\count157}}
\def\@p@@surxb#1{\@urxbtrue \count157=#1 \edef\@p@surxb{\number\count157}}
\def\@p@@suryb#1{\@urybtrue \count157=#1 \edef\@p@suryb{\number\count157}}
\def\@p@@sheightb#1{\@heightbtrue \@whbtrue \count157=#1
	   		\edef\@p@sheightb{\number\count157}}
\def\@p@@swidthb#1{\@widthbtrue \@whbtrue \count157=#1
			\edef\@p@swidthb{\number\count157}}

\def\@p@@sllxc#1{\@llxctrue \count157=#1 \edef\@p@sllxc{\number\count157}}
\def\@p@@sllyc#1{\@llyctrue \count157=#1 \edef\@p@sllyc{\number\count157}}
\def\@p@@surxc#1{\@urxctrue \count157=#1 \edef\@p@surxc{\number\count157}}
\def\@p@@suryc#1{\@uryctrue \count157=#1 \edef\@p@suryc{\number\count157}}
\def\@p@@sheightc#1{\@heightctrue \@whctrue \count157=#1
	   		\edef\@p@sheightc{\number\count157}}
\def\@p@@swidthc#1{\@widthctrue \@whctrue \count157=#1
			\edef\@p@swidthc{\number\count157}}

\def\@p@@sfile#1{\def\@p@sfile{null} 	\openin1=#1
	\ifeof1\typeout{----- FIG ERROR: file #1 not found !!!!!!!!!! }
	\else \closein1
		\@pfiletrue \edef\@p@sfile{#1\space\space}
	\fi
}

\def\@p@@sfiled#1{ \def\@p@sfile{null}	\openin1=#1
	\ifeof1\typeout{----- FIG ERROR: file #1 not found !!!!!!!!!! }
	\else \closein1
		\@pfiletrue \edef\@p@sfile{#1\space\space}
	\fi
}

\def\@p@@sfilea#1{\def\@p@sfilea{null}	\openin1=#1
	\ifeof1\typeout{----- FIG ERROR: file #1 not found !!!!!!!!!! }
	\else \closein1
		\@pfileatrue	\edef\@p@sfilea{#1\space\space}
	\fi
}
\def\@p@@sfileb#1{\def\@p@sfileb{null}	\openin1=#1
	\ifeof1\typeout{----- FIG ERROR: file #1 not found !!!!!!!!!! }
	\else \closein1
		\@pfilebtrue \edef\@p@sfileb{#1\space\space}
	\fi
}
\def\@p@@sfilec#1{\def\@p@sfilec{null}	\openin1=#1
	\ifeof1\typeout{----- FIG ERROR: file #1 not found !!!!!!!!!!}
	\else \closein1
		\@pfilectrue \edef\@p@sfilec{#1\space\space}
	\fi
}
%%
\def\@p@@shsep#1{\@hsepdtrue \count157=#1 \edef\@p@hsep{\number\count157}}
\def\@p@@svsep#1{\@vsepdtrue \count157=#1 \edef\@p@vsep{\number\count157}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newif\ifno@bb \newif\ifno@bba \newif\ifno@bbb 
\newif\ifno@bbc \newif\ifnot@eof
\newread\ps@stream
%
\def\bb@search{
	\typeout{----- FIG: searching \@p@sfile \space for BoundingBox. }
	\openin\ps@stream=\@p@sfile
	\no@bbtrue  \not@eoftrue
	\catcode`\%=12
	\loop
		\read\ps@stream to \line@in
		\global\toks200=\expandafter{\line@in}
		\ifeof\ps@stream \not@eoffalse \fi
		\@bbtest{\toks200}
		\if@bbmatch\not@eoffalse\expandafter\bb@cull\the\toks200\fi
	\ifnot@eof \repeat
	\catcode`\%=14
}
\def\bb@searcha{
%	\typeout{----- FIG: searching \@p@sfilea \space for BoundingBox. }
	\openin\ps@stream=\@p@sfilea
	\no@bbatrue  \not@eoftrue
	\catcode`\%=12
	\loop
		\read\ps@stream to \line@in
		\global\toks200=\expandafter{\line@in}
		\ifeof\ps@stream \not@eoffalse \fi
		\@bbtest{\toks200}
		\if@bbmatch\not@eoffalse\expandafter\bb@culla\the\toks200\fi
	\ifnot@eof \repeat
	\catcode`\%=14
}
\def\bb@searchb{
%	\typeout{----- FIG: searching \@p@sfileb \space  for BoundingBox. }
	\openin\ps@stream=\@p@sfileb
	\no@bbbtrue  \not@eoftrue
	\catcode`\%=12
	\loop
		\read\ps@stream to \line@in
		\global\toks200=\expandafter{\line@in}
		\ifeof\ps@stream \not@eoffalse \fi
		\@bbtest{\toks200}
		\if@bbmatch\not@eoffalse\expandafter\bb@cullb\the\toks200\fi
	\ifnot@eof \repeat
	\catcode`\%=14
}
\def\bb@searchc{
%	\typeout{----- FIG: searching \@p@sfilec \space  for BoundingBox. }
	\openin\ps@stream=\@p@sfilec
	\no@bbctrue  \not@eoftrue
	\catcode`\%=12
	\loop
		\read\ps@stream to \line@in
		\global\toks200=\expandafter{\line@in}
		\ifeof\ps@stream \not@eoffalse \fi
		\@bbtest{\toks200}
		\if@bbmatch\not@eoffalse\expandafter\bb@cullc\the\toks200\fi
	\ifnot@eof \repeat
	\catcode`\%=14
}

%
\catcode`\%=12
\newif\if@bbmatch
\def\@bbtest#1{\expandafter\@a@\the#1%%BoundingBox:\@bbtest\@a@}
\long\def\@a@#1%%BoundingBox:#2#3\@a@{\ifx\@bbtest#2\@bbmatchfalse\else\@bbmatchtrue\fi}
\long\def\bb@cull#1 #2 #3 #4 #5 {
     \count157=#2 \in@difference{\count157}{7} \edef\@p@sllx{\number\@result}
     \count157=#3 \in@difference{\count157}{7} \edef\@p@slly{\number\@result}
     \count157=#4 \in@sum{\count157}{7} \edef\@p@surx{\number\@result}
     \count157=#5 \in@sum{\count157}{7} \edef\@p@sury{\number\@result}
     \no@bbfalse
}
\long\def\bb@culla#1 #2 #3 #4 #5 {
     \count157=#2 \in@difference{\count157}{7} \edef\@p@sllxa{\number\@result}
     \count157=#3 \in@difference{\count157}{7} \edef\@p@sllya{\number\@result}
     \count157=#4 \in@sum{\count157}{7} \edef\@p@surxa{\number\@result}
     \count157=#5 \in@sum{\count157}{7} \edef\@p@surya{\number\@result}
     \no@bbafalse
}
\long\def\bb@cullb#1 #2 #3 #4 #5 {
     \count157=#2 \in@difference{\count157}{7} \edef\@p@sllxb{\number\@result}
     \count157=#3 \in@difference{\count157}{7} \edef\@p@sllyb{\number\@result}
     \count157=#4 \in@sum{\count157}{7} \edef\@p@surxb{\number\@result}
     \count157=#5 \in@sum{\count157}{7} \edef\@p@suryb{\number\@result}
     \no@bbbfalse
}
\long\def\bb@cullc#1 #2 #3 #4 #5 {
     \count157=#2 \in@difference{\count157}{7} \edef\@p@sllxc{\number\@result}
     \count157=#3 \in@difference{\count157}{7} \edef\@p@sllyc{\number\@result}
     \count157=#4 \in@sum{\count157}{7} \edef\@p@surxc{\number\@result}
     \count157=#5 \in@sum{\count157}{7} \edef\@p@suryc{\number\@result}
     \no@bbcfalse
}
\catcode`\%=14
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ps@init@parms{
		\@twofigfalse \@threefigfalse \@threefigabfalse
		\@threefigbafalse \@fourfigfalse
		\@whfalse \@whafalse \@whbfalse \@whcfalse
		\@hsepdfalse \@vsepdfalse
		\no@bbfalse  \no@bbafalse \no@bbbfalse \no@bbcfalse
		\@llxfalse \@llyfalse
		\@urxfalse \@uryfalse
		\@heightfalse \@widthfalse \@pfilefalse
		\def\@p@sllx{}\def\@p@slly{}
		\def\@p@surx{}\def\@p@sury{}
		\def\@p@sheight{}\def\@p@swidth{}
		\def\@p@sfile{} 
		\@llxafalse \@llyafalse
		\@urxafalse \@uryafalse
		\@heightafalse \@widthafalse \@pfileafalse
		\def\@p@sllxa{}\def\@p@sllya{}
		\def\@p@surxa{}\def\@p@surya{}
		\def\@p@sheighta{}\def\@p@swidtha{}
		\def\@p@sfile{} 
		\@llxbfalse \@llybfalse
		\@urxbfalse \@urybfalse 
		\@heightbfalse \@widthbfalse \@pfilebfalse
		\def\@p@sllxb{}\def\@p@sllyb{}
		\def\@p@surxb{}\def\@p@suryb{}
		\def\@p@sheightb{}\def\@p@swidthb{}
		\def\@p@sfileb{}
		\@llxcfalse \@llycfalse
		\@urxcfalse \@urycfalse
		\@heightcfalse \@widthcfalse \@pfilecfalse
		\def\@p@sllxc{}\def\@p@sllyc{}
		\def\@p@surxc{}\def\@p@suryc{}
		\def\@p@sheightc{}\def\@p@swidthc{}
		\def\@p@sfilec{}
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\check@par{ 
		\if@llx \else \no@bbtrue \fi
		\if@lly \else \no@bbtrue \fi
		\if@urx \else \no@bbtrue \fi
		\if@ury \else \no@bbtrue \fi
		\ifno@bb \bb@search \fi
                \ifno@bb  \if@pfile  \if@nobbwarn \else
		     \typeout{----- FIG warning: incomplete BoundingBox !} 
		     \@nobbwarntrue \fi \fi
		     \if@llx \else  \edef\@p@sllx{0} \fi
	  	     \if@lly \else  \edef\@p@slly{0} \fi
		     \if@urx \else  \edef\@p@surx{612} \fi
		     \if@ury \else  \edef\@p@sury{792} \fi
		\fi
		\if@wh \else    % neither of width nor height are defined
				% define width and compute height later
				% according to the aspect ratio
			\@widthtrue 
			\if@fourfig  \edef\@p@swidth{72} 
			\else \edef\@p@swidth{250} \fi
		\fi
% 
\if@height \if@width \else
    \in@compdim{\@p@sllx}{\@p@surx}{\@p@slly}{\@p@sury}{\@p@sheight}
    \edef\@p@swidth{\number\@result} \fi
\fi
\if@width \if@height \else
    \in@compdim{\@p@slly}{\@p@sury}{\@p@sllx}{\@p@surx}{\@p@swidth}
    \edef\@p@sheight{\number\@result} \fi
\fi

\if@pfile
	\if@wh \else \if@nowhwarn \else \@nowhwarntrue
\typeout{----- FIG warning: neither `width(?)' nor `height(?)' are defined !}
	     \fi
	\fi
\fi
}
\def\check@para{ 
		\if@llxa \else \no@bbatrue \fi
		\if@llya \else \no@bbatrue \fi
		\if@urxa \else \no@bbatrue \fi
		\if@urya \else \no@bbatrue \fi
		\ifno@bba \bb@searcha \fi
                \ifno@bba  \if@pfilea \if@nobbwarn \else
		     \typeout{----- FIG warning: incomplete BoundingBox !} 
		     \@nobbwarntrue  \fi \fi
		     \if@llxa \else \edef\@p@sllxa{0} \fi
		     \if@llya \else \edef\@p@sllya{0} \fi
		     \if@urxa \else \edef\@p@surxa{612}\fi
		     \if@urya \else \edef\@p@surya{792}\fi
		\fi
		\if@wha \else \@widthatrue 
			\if@twofig \edef\@p@swidtha{165} \fi
			\if@threefig \edef\@p@swidtha{107} \fi
			\if@threefigab \edef\@p@swidtha{165} \fi
			\if@threefigba \edef\@p@swidtha{165} \fi
			\if@fourfig \edef\@p@swidtha{72} \fi
		\fi
\if@heighta \if@widtha \else
    \in@compdim{\@p@sllxa}{\@p@surxa}{\@p@sllya}{\@p@surya}{\@p@sheighta}
    \edef\@p@swidtha{\number\@result} \fi
\fi
\if@widtha \if@heighta \else
    \in@compdim{\@p@sllya}{\@p@surya}{\@p@sllxa}{\@p@surxa}{\@p@swidtha}
    \edef\@p@sheighta{\number\@result} \fi
\fi

\if@pfilea 
	\if@wha \else \if@nowhwarn \else \@nowhwarntrue
  \typeout{----- FIG warning: neither `widtha' nor `heighta' are defined ! }
       	      \fi 
	\fi
\fi
}
\def\check@parb{ 
		\if@llxb \else \no@bbbtrue \fi
		\if@llyb \else \no@bbbtrue \fi
		\if@urxb \else \no@bbbtrue \fi
		\if@uryb \else \no@bbbtrue \fi
		\ifno@bbb \bb@searchb \fi
                \ifno@bbb \if@pfileb  \if@nobbwarn \else
		     \typeout{----- FIG warning: incomplete BoundingBox !} 
		     \@nobbwarntrue  \fi  \fi
		     \if@llxb \else \edef\@p@sllxb{0} \fi
		     \if@llyb \else \edef\@p@sllyb{0} \fi
		     \if@urxb \else \edef\@p@surxb{612} \fi
		     \if@uryb \else \edef\@p@suryb{792} \fi
		\fi
		\if@whb \else \@widthbtrue
			\if@twofig \edef\@p@swidthb{165} \fi
			\if@threefig \edef\@p@swidthb{107} \fi
			\if@threefigab \edef\@p@swidthb{165} \fi
			\if@threefigba \edef\@p@swidthb{165} \fi
			\if@fourfig \edef\@p@swidthb{72} \fi
		\fi
\if@heightb \if@widthb \else
    \in@compdim{\@p@sllxb}{\@p@surxb}{\@p@sllyb}{\@p@suryb}{\@p@sheightb}
    \edef\@p@swidthb{\number\@result} \fi
\fi
\if@widthb \if@heightb \else
    \in@compdim{\@p@sllyb}{\@p@suryb}{\@p@sllxb}{\@p@surxb}{\@p@swidthb}
    \edef\@p@sheightb{\number\@result} \fi
\fi

\if@pfileb
	\if@whb \else \if@nowhwarn \else \@nowhwarntrue
  \typeout{----- FIG warning: neither `widthb' nor `heightb' are defined ! }
	      \fi 
	\fi
\fi
}
\def\check@parc{ 
		\if@llxc \else \no@bbctrue \fi
		\if@llyc \else \no@bbctrue \fi
		\if@urxc \else \no@bbctrue \fi
		\if@uryc \else \no@bbctrue \fi
		\ifno@bbc \bb@searchc \fi
                \ifno@bbc  \if@pfilec  \if@nobbwarn \else   
		     \typeout{----- FIG warning: incomplete BoundingBox !} 
		     \@nobbwarntrue  \fi \fi
		     \if@llxc \else \edef\@p@sllxc{0} \fi
		     \if@llyc \else \edef\@p@sllyc{0} \fi
		     \if@urxc \else \edef\@p@surxc{612} \fi
		     \if@uryc \else \edef\@p@suryc{792} \fi
		\fi
		\if@whc \else \@widthctrue
			\if@threefig \edef\@p@swidthc{100} \fi
			\if@threefigab \edef\@p@swidthc{165} \fi
			\if@threefigba \edef\@p@swidthc{165} \fi
			\if@fourfig \edef\@p@swidthc{72} \fi
		\fi
\if@heightc \if@widthc \else
    \in@compdim{\@p@sllxc}{\@p@surxc}{\@p@sllyc}{\@p@suryc}{\@p@sheightc}
    \edef\@p@swidthc{\number\@result} \fi
\fi
\if@widthc \if@heightc \else
    \in@compdim{\@p@sllyc}{\@p@suryc}{\@p@sllxc}{\@p@surxc}{\@p@swidthc}
    \edef\@p@sheightc{\number\@result} \fi
\fi

\if@pfilec 
	\if@whc \else \if@nowhwarn \else \@nowhwarntrue 
 \typeout{----- FIG warning: neither `widthc' nor `heightc' are defined ! }
      	     \fi 
	\fi
\fi
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\check@sep{
   \if@hsepd
	\if@twofig \edef\@hsep{\number\@p@hsep} \fi
	\if@threefigab \edef\@hsep{\number\@p@hsep} \fi
	\if@threefigba \edef\@hsep{\number\@p@hsep} \fi
	\if@threefig  
		\edef\@hsep{\number\@p@hsep} 
		\in@times{\@p@hsep}{2} \edef\@dhsep{\number\@result} 
	\fi
	\if@fourfig  
		\edef\@hsep{\number\@p@hsep} 
		\in@times{\@p@hsep}{2} \edef\@dhsep{\number\@result} 
		\in@times{\@p@hsep}{3} \edef\@thsep{\number\@result} 
	\fi
   \fi
   \if@vsepd  \edef\@vsep{\number\@p@vsep} \fi
}		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% OneFigure Macro
%
\def\OneFigure#1#2{
	\ps@init@parms
	\parse@ps@parms{#1}
	\check@par

	\in@difference{\@p@surx}{\@p@sllx} \edef\@twidth{\number\@result}
	\in@difference{\@p@sury}{\@p@slly} \edef\@theight{\number\@result}
	\in@atbdc{\@p@swidth}{100}{\@twidth}
		\edef\@xscale{\number\@result\space\space}
	\in@atbdc{\@p@sheight}{100}{\@theight}
		\edef\@yscale{\number\@result\space\space}
	\in@atbdc{\@p@sllx}{\@xscale}{-100}
		 \edef\@xoff{\number\@result\space\space}
	\in@atbdc{\@p@slly}{\@yscale}{-100}
		 \edef\@yoff{\number\@result\space\space}
%
%   Give warning when the figures are too wide.
%
\dimen0=\@p@swidth pt	
\ifdim \dimen0 >\hsize
	\typeout{----- OneFigure warning: ps figure is too wide ! }
\fi
%

%
	\vskip 10pt \nobreak
	\hbox to \hsize{
		\hss
		\dimen0= \@p@swidth pt
		\hbox to \dimen0 {
			\dimen0= \@p@sheight pt
			\vbox to \dimen0{
					\vss
					\special{psfile=\@p@sfile
						hoffset=\@xoff
						voffset=\@yoff
						hscale=\@xscale 
						vscale=\@yscale }
					}
					\hss
				}
			\hss
		}
	\vskip 6pt \nobreak
	\centerline{#2}
	\vskip 4pt
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TwoFigures Macro
%
\def\TwoFigures#1#2#3{
	\ps@init@parms
	\@twofigtrue  \edef\@hsep{36}
	\parse@ps@parms{#1} 
	\parse@ps@parms{#2}
	\check@para 
	\check@parb
 	\check@sep

	\in@difference{\@p@surxa}{\@p@sllxa} \edef\@twidtha{\number\@result}
	\in@difference{\@p@surya}{\@p@sllya} \edef\@theighta{\number\@result}
	\in@atbdc{\@p@swidtha}{100}{\@twidtha}
		\edef\@xscalea{\number\@result\space\space}
	\in@atbdc{\@p@sheighta}{100}{\@theighta}
		\edef\@yscalea{\number\@result\space\space}
	\in@difference{\@p@surxb}{\@p@sllxb} \edef\@twidthb{\number\@result}
	\in@difference{\@p@suryb}{\@p@sllyb} \edef\@theightb{\number\@result}
	\in@atbdc{\@p@swidthb}{100}{\@twidthb}
		\edef\@xscaleb{\number\@result\space\space}
	\in@atbdc{\@p@sheightb}{100}{\@theightb}
		\edef\@yscaleb{\number\@result\space\space}

	\in@sum{\@p@swidtha}{\@p@swidthb} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@hsep} \edef\@hsizee{\number\@result\space}

	\in@times{\@p@sllxa}{-1}
		 \edef\@xoffa{\number\@result\space\space}
	\in@times{\@p@sllxb}{-1}
		 \edef\@xoffbt{\number\@result}

	\in@difference{\@p@swidtha}{\@p@swidthb} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@hsep} \edef\@fdifw{\number\@result}
	\in@times{\@p@swidthb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifw}{\@twidthb}{\@tmpa} \edef\@fdifww{\number\@result}
	\in@sum{\@fdifww}{\@xoffbt}
		\edef\@xoffb{\number\@result\space\space\space}

	\in@times{\@p@sllya}{-1}
		 \edef\@yoffat{\number\@result\space\space}
	\in@times{\@p@sllyb}{-1}
		 \edef\@yoffbt{\number\@result\space\space}
	\in@max{\@p@sheighta}{\@p@sheightb}{0}
		\edef\@maxh{\number\@result}

	\in@difference{\@maxh}{\@p@sheighta}\edef\@tmp{\number\@result}
	\in@times{\@p@sheighta}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@theighta}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffat}
		\edef\@yoffa{\number\@result\space\space}

	\in@difference{\@maxh}{\@p@sheightb} \edef\@tmp{\number\@result}
	\in@times{\@p@sheightb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@theightb}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffbt}
		\edef\@yoffb{\number\@result\space\space}
	\in@atbdc{\@xoffa}{\@xscalea}{100} \edef\@xoffa{\number\@result\space\space}
	\in@atbdc{\@xoffb}{\@xscaleb}{100} \edef\@xoffb{\number\@result\space\space}
	\in@atbdc{\@yoffa}{\@yscalea}{100} \edef\@yoffa{\number\@result\space\space}
	\in@atbdc{\@yoffb}{\@yscaleb}{100} \edef\@yoffb{\number\@result\space\space}
%
%   Give warning when the figures are too wide.
%
\dimen0=\@hsizee pt	
\ifdim \dimen0 >\hsize
	\typeout{----- TwoFigures warning: ps figures are too wide ! }
\fi
%
	\vskip 10pt \nobreak
	\hbox to \hsize{
		\hss
		\dimen0= \@hsizee pt
		\hbox to \dimen0 {
			\dimen0= \@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfilea }
					\special{psfile=\@p@sfilea
						hoffset = \@xoffa
						voffset = \@yoffa
						hscale=\@xscalea 
						vscale=\@yscalea}
					 }
					\hss
			\dimen0=\@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfileb }
					\special{psfile=\@p@sfileb
						hoffset = \@xoffb
						voffset = \@yoffb
						hscale=\@xscaleb 
						vscale=\@yscaleb}
					}
					\hss
				}
			\hss
		}
	\vskip 6pt \nobreak
	\centerline{#3}
	\vskip 4pt
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ThreeFigures Macro
%
\def\ThreeFigures#1#2#3#4{
	\ps@init@parms
	\@threefigtrue
	\edef\@hsep{24} \edef\@dhsep{48}
	\parse@ps@parms{#1}
	\parse@ps@parms{#2}
	\parse@ps@parms{#3}
	\check@para
	\check@parb
	\check@parc
	\check@sep
%
% scale factors
%
	\in@difference{\@p@surxa}{\@p@sllxa} \edef\@twidtha{\number\@result}
	\in@difference{\@p@surya}{\@p@sllya} \edef\@theighta{\number\@result}
	\in@atbdc{\@p@swidtha}{100}{\@twidtha}
		\edef\@xscalea{\number\@result\space\space}
	\in@atbdc{\@p@sheighta}{100}{\@theighta}
		\edef\@yscalea{\number\@result\space\space}
	\in@difference{\@p@surxb}{\@p@sllxb} \edef\@twidthb{\number\@result}
	\in@difference{\@p@suryb}{\@p@sllyb} \edef\@theightb{\number\@result}
	\in@atbdc{\@p@swidthb}{100}{\@twidthb}
		\edef\@xscaleb{\number\@result\space\space}
	\in@atbdc{\@p@sheightb}{100}{\@theightb}
		\edef\@yscaleb{\number\@result\space\space}
	\in@difference{\@p@surxc}{\@p@sllxc} \edef\@twidthc{\number\@result}
	\in@difference{\@p@suryc}{\@p@sllyc} \edef\@theightc{\number\@result}
	\in@atbdc{\@p@swidthc}{100}{\@twidthc}
		\edef\@xscalec{\number\@result\space\space}
	\in@atbdc{\@p@sheightc}{100}{\@theightc}
		\edef\@yscalec{\number\@result\space\space}
%
% total hsize
%
	\in@sum{\@p@swidtha}{\@p@swidthb} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@p@swidthc} \edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@dhsep} \edef\@hsizee{\number\@result\space}
%
%  tmp offsets
%
	\in@times{\@p@sllxa}{-1}
		 \edef\@xoffa{\number\@result\space\space}
	\in@times{\@p@sllxb}{-1}
		 \edef\@xoffbt{\number\@result}
	\in@times{\@p@sllxc}{-1}
		 \edef\@xoffct{\number\@result}
	\in@times{\@p@sllya}{-1}
		 \edef\@yoffat{\number\@result\space\space}
	\in@times{\@p@sllyb}{-1}
		 \edef\@yoffbt{\number\@result}
	\in@times{\@p@sllyc}{-1}
		 \edef\@yoffct{\number\@result}
%
% compute offsets
%
%
	\in@times{\@p@swidtha}{2} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@hsep}  \edef\@tmpp{\number\@result}
	\in@difference{\@tmpp}{\@p@swidthb}
			\edef\@tmp{\number\@result}
	\in@difference{\@tmp}{\@p@swidthc}
			\edef\@fdifw{\number\@result}
	\in@times{\@p@swidthb}{3} \edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifw}{\@twidthb}{\@tmpa}
		\edef\@fdifww{\number\@result}
	\in@sum{\@fdifww}{\@xoffbt}
		\edef\@xoffb{\number\@result\space\space\space}

	\in@times{\@p@swidthc}{2} \edef\@tmp{\number\@result}
	\in@difference{\@p@swidtha}{\@tmp} \edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@p@swidthb} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@dhsep} \edef\@fdifw{\number\@result}
	\in@times{\@p@swidthc}{3} \edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifw}{\@twidthc}{\@tmpa}
		\edef\@fdifww{\number\@result}
	\in@sum{\@fdifww}{\@xoffct}
		\edef\@xoffc{\number\@result\space\space\space}


	\in@max{\@p@sheighta}{\@p@sheightb}{\@p@sheightc}
		\edef\@maxh{\number\@result}

	\in@difference{\@maxh}{\@p@sheighta}
		\edef\@fdifh{\number\@result}
	\in@times{\@p@sheighta}{2}\edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifh}{\@theighta}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffat}
		\edef\@yoffa{\number\@result\space\space}

	\in@difference{\@maxh}{\@p@sheightb}
		\edef\@fdihw{\number\@result}
	\in@times{\@p@sheightb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@fdihw}{\@theightb}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffbt}
		\edef\@yoffb{\number\@result\space\space}

	\in@difference{\@maxh}{\@p@sheightc}
		\edef\@fdifh{\number\@result}
	\in@times{\@p@sheightc}{2}  \edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifh}{\@theightc}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffct}
		\edef\@yoffc{\number\@result\space\space}

	\in@atbdc{\@xoffa}{\@xscalea}{100} \edef\@xoffa{\number\@result\space\space}
	\in@atbdc{\@xoffb}{\@xscaleb}{100} \edef\@xoffb{\number\@result\space\space}
	\in@atbdc{\@xoffc}{\@xscalec}{100} \edef\@xoffc{\number\@result\space\space}
	\in@atbdc{\@yoffa}{\@yscalea}{100} \edef\@yoffa{\number\@result\space\space}
	\in@atbdc{\@yoffb}{\@yscaleb}{100} \edef\@yoffb{\number\@result\space\space}
	\in@atbdc{\@yoffc}{\@yscalec}{100} \edef\@yoffc{\number\@result\space\space}
%
%   Give warning when the figures are too wide.
%
\dimen0=\@hsizee pt	
\ifdim \dimen0 >\hsize
	\typeout{----- ThreeFigures warning: ps figures are too wide ! }
\fi
%
	\vskip 10pt \nobreak
	\hbox to \hsize{
		\hss
		\dimen0= \@hsizee pt
		\hbox to \dimen0 {
			\dimen0= \@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfilea }
					\special{psfile=\@p@sfilea
						hoffset = \@xoffa
						voffset = \@yoffa
						hscale=\@xscalea 
						vscale=\@yscalea}
					 }
					\hss
			\dimen0=\@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfileb }
					\special{psfile=\@p@sfileb
						hoffset = \@xoffb
						voffset = \@yoffb
						hscale=\@xscaleb 
						vscale=\@yscaleb}
					}
					\hss
			\dimen0=\@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfilec }
					\special{psfile=\@p@sfilec
						hoffset = \@xoffc
						voffset = \@yoffc
						hscale=\@xscalec
						vscale=\@yscalec}
					}
					\hss
				}
			\hss
		}
	\vskip 6pt \nobreak
	\centerline{#4}
	\vskip 4pt
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ThreeFigures Macro
%
\def\ThreeFiguresAB#1#2#3#4{
	\ps@init@parms
	\@threefigabtrue
	\edef\@hsep{36} \edef\@vsep{20}
	\parse@ps@parms{#1}
	\parse@ps@parms{#2}
	\parse@ps@parms{#3}
	\check@para
	\check@parb
	\check@parc
	\check@sep
%
% scale factors
%
	\in@difference{\@p@surxa}{\@p@sllxa} \edef\@twidtha{\number\@result}
	\in@difference{\@p@surya}{\@p@sllya} \edef\@theighta{\number\@result}
	\in@atbdc{\@p@swidtha}{100}{\@twidtha}
		\edef\@xscalea{\number\@result\space\space}
	\in@atbdc{\@p@sheighta}{100}{\@theighta}
		\edef\@yscalea{\number\@result\space\space}
	\in@difference{\@p@surxb}{\@p@sllxb} \edef\@twidthb{\number\@result}
	\in@difference{\@p@suryb}{\@p@sllyb} \edef\@theightb{\number\@result}
	\in@atbdc{\@p@swidthb}{100}{\@twidthb} 
		\edef\@xscaleb{\number\@result\space\space}
	\in@atbdc{\@p@sheightb}{100}{\@theightb}
		\edef\@yscaleb{\number\@result\space\space}
	\in@difference{\@p@surxc}{\@p@sllxc} \edef\@twidthc{\number\@result}
	\in@difference{\@p@suryc}{\@p@sllyc} \edef\@theightc{\number\@result}
	\in@atbdc{\@p@swidthc}{100}{\@twidthc}
		\edef\@xscalec{\number\@result\space\space}
	\in@atbdc{\@p@sheightc}{100}{\@theightc} 
		\edef\@yscalec{\number\@result\space\space}
%
% total hsize
%
	\in@max{\@p@swidthb}{\@p@swidthc}{0} \edef\@tmp{\number\@result}
	\in@sum{\@p@swidtha}{\@tmp} \edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@hsep} \edef\@hsizee{\number\@result\space}
%
%  tmp offsets
%
	\in@times{\@p@sllxa}{-1}
		 \edef\@xoffa{\number\@result\space\space}
	\in@times{\@p@sllxb}{-1}
		 \edef\@xoffbt{\number\@result}
	\in@times{\@p@sllxc}{-1}
		 \edef\@xoffct{\number\@result}
	\in@times{\@p@sllya}{-1}
		 \edef\@yoffat{\number\@result\space\space}
	\in@times{\@p@sllyb}{-1}
		 \edef\@yoffbt{\number\@result}
	\in@times{\@p@sllyc}{-1}
		 \edef\@yoffct{\number\@result}
%
% tmp dimensions
%
	\in@sum{\@p@sheightb}{\@p@sheightc}
			\edef\@tmp{\number\@result}	
	\in@sum{\@tmp}{\@vsep} \edef\@hbc{\number\@result\space}
	\in@max{\@hbc}{\@p@sheighta}{0} \edef\@maxh{\number\@result}

	\in@max{\@p@swidthb}{\@p@swidthc}{0}
		\edef\@maxwbc{\number\@result}

	\in@difference{\@p@swidtha}{\@maxwbc}
			\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@hsep} \edef\@xoffbct{\number\@result}

%
% compute offsets
%
%
	\in@difference{\@maxwbc}{\@p@swidthb}
			\edef\@tmpp{\number\@result}
	\in@sum{\@xoffbct}{\@tmpp} \edef\@tmp{\number\@result}
	\in@times{\@p@swidthb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@twidthb}{\@tmpa}
		\edef\@tmpp{\number\@result}
	\in@sum{\@xoffbt}{\@tmpp} 
		\edef\@xoffb{\number\@result\space\space\space}

	\in@difference{\@maxwbc}{\@p@swidthc}
			\edef\@tmpp{\number\@result}
	\in@sum{\@xoffbct}{\@tmpp} \edef\@tmp{\number\@result}
	\in@times{\@p@swidthc}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@twidthc}{\@tmpa}
		\edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@xoffct}
		\edef\@xoffc{\number\@result\space\space\space}

	\in@difference{\@maxh}{\@p@sheighta}
		\edef\@tmpp{\number\@result}
	\in@times{\@p@sheighta}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmpp}{\@theighta}{\@tmpa}
		\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@yoffat}
		\edef\@yoffa{\number\@result\space\space}

	\in@difference{\@p@sheightc}{\@p@sheightb}
		\edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@vsep} \edef\@tmpp{\number\@result}
	\in@times{\@p@sheightb}{2} \edef\@tmpa{\number\@result}	
	\in@atbdc{\@tmpp}{\@theightb}{\@tmpa}
		\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@yoffbt}
		\edef\@yoffb{\number\@result\space\space}

	\in@difference{\@maxh}{\@hbc}
		\edef\@tmpp{\number\@result}
	\in@times{\@p@sheightc}{2} \edef\@tmpa{\number\@result}	
	\in@atbdc{\@tmpp}{\@theightc}{\@tmpa}
		\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@yoffct}
		\edef\@yoffc{\number\@result\space\space}

	\in@quotient{\@maxh}{2} \edef\@hmaxh{\number\@quotient}

	\in@atbdc{\@xoffa}{\@xscalea}{100} \edef\@xoffa{\number\@result\space\space}
	\in@atbdc{\@xoffb}{\@xscaleb}{100} \edef\@xoffb{\number\@result\space\space}
	\in@atbdc{\@xoffc}{\@xscalec}{100} \edef\@xoffc{\number\@result\space\space}
	\in@atbdc{\@yoffa}{\@yscalea}{100} \edef\@yoffa{\number\@result\space\space}
	\in@atbdc{\@yoffb}{\@yscaleb}{100} \edef\@yoffb{\number\@result\space\space}
	\in@atbdc{\@yoffc}{\@yscalec}{100} \edef\@yoffc{\number\@result\space\space}
%
%   Give warning when the figures are too wide.
%
\dimen0=\@hsizee pt	
\ifdim \dimen0 >\hsize
	\typeout{----- ThreeFiguresAB warning: ps figures are too wide ! }
\fi
%
	\vskip 10pt \nobreak
	\hbox to \hsize{ 
		\hss
		\dimen0= \@hsizee pt
		\hbox to \dimen0 { 
			\dimen0= \@maxh pt
			\vbox to \dimen0{ 
					\vss
%	\typeout{----- FIG: including \@p@sfilea }
					\special{psfile=\@p@sfilea
						hoffset = \@xoffa
						voffset = \@yoffa
						hscale=\@xscalea 
						vscale=\@yscalea}
					 }
					\hss
			\dimen0=\@maxh pt
			\vbox to \dimen0{
					\vss
					\dimen0 = \@hmaxh pt
					\vbox to \dimen0{ \vss
%	\typeout{----- FIG: including \@p@sfileb }
					\special{psfile=\@p@sfileb
						hoffset = \@xoffb
						voffset = \@yoffb
						hscale=\@xscaleb 
						vscale=\@yscaleb}
					    }
					\dimen0=\@hmaxh pt
					\vbox to \dimen0{\vss
%	\typeout{----- FIG: including \@p@sfilec }
					\special{psfile=\@p@sfilec
						hoffset = \@xoffc
						voffset = \@yoffc
						hscale=\@xscalec
						vscale=\@yscalec}
					}
				}\hss
			   }
			\hss
		}
	\vskip 6pt \nobreak
	\centerline{#4}
	\vskip 4pt
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ThreeFigures Macro
%
\def\ThreeFiguresBA#1#2#3#4{
	\ps@init@parms
	\@threefigbatrue
	\edef\@hsep{36} \edef\@vsep{20}
	\parse@ps@parms{#1}
	\parse@ps@parms{#2}
	\parse@ps@parms{#3}
	\check@para
	\check@parb
	\check@parc
	\check@sep
%
% scale factors
%
	\in@difference{\@p@surxa}{\@p@sllxa} \edef\@twidtha{\number\@result}
	\in@difference{\@p@surya}{\@p@sllya} \edef\@theighta{\number\@result}
	\in@atbdc{\@p@swidtha}{100}{\@twidtha} 
		\edef\@xscalea{\number\@result\space\space}
	\in@atbdc{\@p@sheighta}{100}{\@theighta}
		\edef\@yscalea{\number\@result\space\space}
	\in@difference{\@p@surxb}{\@p@sllxb} \edef\@twidthb{\number\@result}
	\in@difference{\@p@suryb}{\@p@sllyb} \edef\@theightb{\number\@result}
	\in@atbdc{\@p@swidthb}{100}{\@twidthb} 
		\edef\@xscaleb{\number\@result\space\space}
	\in@atbdc{\@p@sheightb}{100}{\@theightb}
		\edef\@yscaleb{\number\@result\space\space}
	\in@difference{\@p@surxc}{\@p@sllxc} \edef\@twidthc{\number\@result}
	\in@difference{\@p@suryc}{\@p@sllyc} \edef\@theightc{\number\@result}
	\in@atbdc{\@p@swidthc}{100}{\@twidthc}
		\edef\@xscalec{\number\@result\space\space}
	\in@atbdc{\@p@sheightc}{100}{\@theightc} 
		\edef\@yscalec{\number\@result\space\space}
%
% total hsize
%
	\in@max{\@p@swidtha}{\@p@swidthb}{0} \edef\@tmp{\number\@result}
	\in@sum{\@p@swidthc}{\@tmp} \edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@hsep} \edef\@hsizee{\number\@result\space}
%
%  tmp offsets
%
	\in@times{\@p@sllxa}{-1}
		 \edef\@xoffat{\number\@result\space\space}
	\in@times{\@p@sllxb}{-1}
		 \edef\@xoffbt{\number\@result}
	\in@times{\@p@sllxc}{-1}
		 \edef\@xoffct{\number\@result}
	\in@times{\@p@sllya}{-1}
		 \edef\@yoffat{\number\@result\space\space}
	\in@times{\@p@sllyb}{-1}
		 \edef\@yoffbt{\number\@result}
	\in@times{\@p@sllyc}{-1}
		 \edef\@yoffct{\number\@result}
%
% tmp dimensions
%
	\in@sum{\@p@sheighta}{\@p@sheightb}
			\edef\@tmp{\number\@result}	
	\in@sum{\@tmp}{\@vsep} \edef\@hab{\number\@result\space}
	\in@max{\@hab}{\@p@sheightc}{0} \edef\@maxh{\number\@result}

	\in@max{\@p@swidtha}{\@p@swidthb}{0}
		\edef\@maxwab{\number\@result}

%
% compute offsets
%
%
	\in@difference{\@maxwab}{\@p@swidtha}
			\edef\@tmp{\number\@result}
	\in@times{\@p@swidtha}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@twidtha}{\@tmpa}
		\edef\@tmpp{\number\@result}
	\in@sum{\@xoffat}{\@tmpp} 
		\edef\@xoffa{\number\@result\space\space\space}

	\in@difference{\@maxwab}{\@p@swidthb}
			\edef\@tmp{\number\@result}
	\in@times{\@p@swidthb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@twidthb}{\@tmpa}
		\edef\@tmpp{\number\@result}
	\in@sum{\@xoffbt}{\@tmpp} 
		\edef\@xoffb{\number\@result\space\space\space}

	\in@difference{\@maxwab}{\@p@swidthc}
			\edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@hsep} \edef\@tmp{\number\@result}
	\in@times{\@p@swidthc}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@twidthc}{\@tmpa}
		\edef\@tmpp{\number\@result}
	\in@sum{\@xoffct}{\@tmpp} 
		\edef\@xoffc{\number\@result\space\space\space}

	\in@difference{\@maxh}{\@p@sheightc}
		\edef\@tmpp{\number\@result}
	\in@times{\@p@sheightc}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmpp}{\@theightc}{\@tmpa}
		\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@yoffct}
		\edef\@yoffc{\number\@result\space\space}

	\in@difference{\@maxh}{\@hab}
		\edef\@tmpp{\number\@result}
	\in@times{\@p@sheightb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmpp}{\@theightb}{\@tmpa}
		\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@yoffbt}
		\edef\@yoffb{\number\@result\space\space}

	\in@difference{\@p@sheightb}{\@p@sheighta}
		\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@vsep} \edef\@tmpp{\number\@result}
	\in@times{\@p@sheighta}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmpp}{\@theighta}{\@tmpa}
		\edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@yoffat}
		\edef\@yoffa{\number\@result\space\space}

	\in@quotient{\@maxh}{2} \edef\@hmaxh{\number\@quotient}

	\in@atbdc{\@xoffa}{\@xscalea}{100} \edef\@xoffa{\number\@result\space\space}
	\in@atbdc{\@xoffb}{\@xscaleb}{100} \edef\@xoffb{\number\@result\space\space}
	\in@atbdc{\@xoffc}{\@xscalec}{100} \edef\@xoffc{\number\@result\space\space}
	\in@atbdc{\@yoffa}{\@yscalea}{100} \edef\@yoffa{\number\@result\space\space}
	\in@atbdc{\@yoffb}{\@yscaleb}{100} \edef\@yoffb{\number\@result\space\space}
	\in@atbdc{\@yoffc}{\@yscalec}{100} \edef\@yoffc{\number\@result\space\space}
%
%   Give warning when the figures are too wide.
%
\dimen0=\@hsizee pt	
\ifdim \dimen0 >\hsize
	\typeout{----- ThreeFiguresBA warning: ps figures are too wide ! }
\fi
%
	\vskip 10pt \nobreak
	\hbox to \hsize{ 
		\hss
		\dimen0= \@hsizee pt
		\hbox to \dimen0 { 
			\dimen0=\@maxh pt
			\vbox to \dimen0{
					\vss
					\dimen0 = \@hmaxh pt
					\vbox to \dimen0{ \vss
%	\typeout{----- FIG: including \@p@sfilea }
					\special{psfile=\@p@sfilea
						hoffset = \@xoffa
						voffset = \@yoffa
						hscale=\@xscalea 
						vscale=\@yscalea}
					    }
					\dimen0=\@hmaxh pt
					\vbox to \dimen0{\vss
%	\typeout{----- FIG: including \@p@sfileb }
					\special{psfile=\@p@sfileb
						hoffset = \@xoffb
						voffset = \@yoffb
						hscale=\@xscaleb
						vscale=\@yscaleb}
					}
				}\hss
			\dimen0= \@maxh pt
			\vbox to \dimen0{ 
					\vss
%	\typeout{----- FIG: including \@p@sfilec }
					\special{psfile=\@p@sfilec
						hoffset = \@xoffc
						voffset = \@yoffc
						hscale=\@xscalec
						vscale=\@yscalec}
					 }
					\hss

			   }
			\hss
		}
	\vskip 6pt \nobreak
	\centerline{#4}
	\vskip 4pt
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Optional FourFigures Macro. Align four figures horizontally.
%
%
\def\FourFigures#1#2#3#4#5{
	\ps@init@parms
	\@fourfigtrue
	\edef\@hsep{16} \edef\@dhsep{32} \edef\@thsep{48}
	\parse@ps@parms{#1}
	\parse@ps@parms{#2}
	\parse@ps@parms{#3}
	\parse@ps@parms{#4}
	\check@par
	\check@para
	\check@parb
	\check@parc
	\check@sep
%
% switch      a b c d      to       d a b c == 1 2 3 4
%	
\edef\@tmpllx{\number\@p@sllx}
\edef\@tmplly{\number\@p@slly}
\edef\@tmpurx{\number\@p@surx}
\edef\@tmpury{\number\@p@sury}
\edef\@tmpwidth{\number\@p@swidth}
\edef\@tmpheight{\number\@p@sheight}
\edef\@tmpfile{\@p@sfile}

\edef\@p@sllx{\number\@p@sllxa}
\edef\@p@sllxa{\number\@p@sllxb}
\edef\@p@sllxb{\number\@p@sllxc}
\edef\@p@sllxc{\number\@tmpllx}

\edef\@p@slly{\number\@p@sllya}
\edef\@p@sllya{\number\@p@sllyb}
\edef\@p@sllyb{\number\@p@sllyc}
\edef\@p@sllyc{\number\@tmplly}

\edef\@p@surx{\number\@p@surxa}
\edef\@p@surxa{\number\@p@surxb}
\edef\@p@surxb{\number\@p@surxc}
\edef\@p@surxc{\number\@tmpurx}

\edef\@p@sury{\number\@p@surya}
\edef\@p@surya{\number\@p@suryb}
\edef\@p@suryb{\number\@p@suryc}
\edef\@p@suryc{\number\@tmpury}

\edef\@p@swidth{\number\@p@swidtha}
\edef\@p@swidtha{\number\@p@swidthb}
\edef\@p@swidthb{\number\@p@swidthc}
\edef\@p@swidthc{\number\@tmpwidth}


\edef\@p@sheight{\number\@p@sheighta}
\edef\@p@sheighta{\number\@p@sheightb}
\edef\@p@sheightb{\number\@p@sheightc}
\edef\@p@sheightc{\number\@tmpheight}

\edef\@p@sfile{\@p@sfilea}
\edef\@p@sfilea{\@p@sfileb}
\edef\@p@sfileb{\@p@sfilec}
\edef\@p@sfilec{\@tmpfile}

%
% end of switches

%
% scale factors
%
	\in@difference{\@p@surx}{\@p@sllx} \edef\@twidth{\number\@result}
	\in@difference{\@p@sury}{\@p@slly} \edef\@theight{\number\@result}
	\in@atbdc{\@p@swidth}{100}{\@twidth}
		\edef\@xscale{\number\@result\space\space}
	\in@atbdc{\@p@sheight}{100}{\@theight}
		\edef\@yscale{\number\@result\space\space}
	\in@difference{\@p@surxa}{\@p@sllxa} \edef\@twidtha{\number\@result}
	\in@difference{\@p@surya}{\@p@sllya} \edef\@theighta{\number\@result}
	\in@atbdc{\@p@swidtha}{100}{\@twidtha}
		\edef\@xscalea{\number\@result\space\space}
	\in@atbdc{\@p@sheighta}{100}{\@theighta}
		\edef\@yscalea{\number\@result\space\space}
	\in@difference{\@p@surxb}{\@p@sllxb} \edef\@twidthb{\number\@result}
	\in@difference{\@p@suryb}{\@p@sllyb} \edef\@theightb{\number\@result}
	\in@atbdc{\@p@swidthb}{100}{\@twidthb} 	
		\edef\@xscaleb{\number\@result\space\space}
	\in@atbdc{\@p@sheightb}{100}{\@theightb}
		\edef\@yscaleb{\number\@result\space\space}
	\in@difference{\@p@surxc}{\@p@sllxc} \edef\@twidthc{\number\@result}
	\in@difference{\@p@suryc}{\@p@sllyc} \edef\@theightc{\number\@result}
	\in@atbdc{\@p@swidthc}{100}{\@twidthc}
		\edef\@xscalec{\number\@result\space\space}
	\in@atbdc{\@p@sheightc}{100}{\@theightc}
		\edef\@yscalec{\number\@result\space\space}
%
% total hsize
%
	\in@sum{\@p@swidth}{\@p@swidtha} \edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@p@swidthb} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@p@swidthc} \edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@thsep} \edef\@hsizee{\number\@result\space}
%
%  tmp offsets
%
	\in@times{\@p@sllx}{-1}
		 \edef\@xoff{\number\@result\space\space}
	\in@times{\@p@sllxa}{-1}
		 \edef\@xoffat{\number\@result\space\space}
	\in@times{\@p@sllxb}{-1}
		 \edef\@xoffbt{\number\@result}
	\in@times{\@p@sllxc}{-1}
		 \edef\@xoffct{\number\@result}
	\in@times{\@p@slly}{-1}
		 \edef\@yofft{\number\@result\space\space}
	\in@times{\@p@sllya}{-1}
		 \edef\@yoffat{\number\@result\space\space}
	\in@times{\@p@sllyb}{-1}
		 \edef\@yoffbt{\number\@result}
	\in@times{\@p@sllyc}{-1}
		 \edef\@yoffct{\number\@result}
%
% compute offsets
%
%
	\in@sum{\@p@swidth}{\@hsep} \edef\@tmp{\number\@result}
	\in@times{\@tmp}{4}  \edef\@tmpp{\number\@result}
	\in@difference{\@tmpp}{\@hsizee} \edef\@tmp{\number\@result}
	\in@times{\@p@swidtha}{4} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmp}{\@twidtha}{\@tmpa}
		\edef\@fdifww{\number\@result}
	\in@sum{\@fdifww}{\@xoffat}
		\edef\@xoffa{\number\@result\space\space\space}

	\in@sum{\@p@swidth}{\@p@swidtha} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@dhsep} \edef\@tmpp{\number\@result}
	\in@times{\@tmpp}{2} \edef\@tmp{\number\@result}
	\in@difference{\@tmp}{\@hsizee} \edef\@tmpp{\number\@result}
	\in@times{\@p@swidthb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmpp}{\@twidthb}{\@tmpa}
		\edef\@fdifww{\number\@result}
	\in@sum{\@fdifww}{\@xoffbt}
		\edef\@xoffb{\number\@result\space\space\space}

	\in@sum{\@p@swidth}{\@p@swidtha} \edef\@tmp{\number\@result}
	\in@sum{\@tmp}{\@p@swidthb} \edef\@tmpp{\number\@result}
	\in@sum{\@tmpp}{\@thsep} \edef\@tmp{\number\@result}
	\in@times{\@tmp}{4} \edef\@tmpp{\number\@result}
	\in@times{\@hsizee}{3} \edef\@tmp{\number\@result}	
	\in@difference{\@tmpp}{\@tmp} \edef\@tmpp{\number\@result}
	\in@times{\@p@swidthc}{4} \edef\@tmpa{\number\@result}
	\in@atbdc{\@tmpp}{\@twidthc}{\@tmpa}
		\edef\@fdifww{\number\@result}
	\in@sum{\@fdifww}{\@xoffct}
		\edef\@xoffc{\number\@result\space\space\space}


	\in@max{\@p@sheighta}{\@p@sheightb}{\@p@sheightc}
		\edef\@tmp{\number\@result}
	\in@max{\@tmp}{\@p@sheight}{0}
		\edef\@maxh{\number\@result}

	\in@difference{\@maxh}{\@p@sheight}
		\edef\@fdifh{\number\@result}
	\in@times{\@p@sheight}{2}\edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifh}{\@theight}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yofft}
		\edef\@yoff{\number\@result\space\space}

	\in@difference{\@maxh}{\@p@sheighta}
		\edef\@fdifh{\number\@result}
	\in@times{\@p@sheighta}{2}\edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifh}{\@theighta}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffat}
		\edef\@yoffa{\number\@result\space\space}

	\in@difference{\@maxh}{\@p@sheightb}
		\edef\@fdihw{\number\@result}
	\in@times{\@p@sheightb}{2} \edef\@tmpa{\number\@result}
	\in@atbdc{\@fdihw}{\@theightb}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffbt}
		\edef\@yoffb{\number\@result\space\space}

	\in@difference{\@maxh}{\@p@sheightc}
		\edef\@fdifh{\number\@result}
	\in@times{\@p@sheightc}{2}  \edef\@tmpa{\number\@result}
	\in@atbdc{\@fdifh}{\@theightc}{\@tmpa}
		\edef\@fdifhh{\number\@result}
	\in@sum{\@fdifhh}{\@yoffct}
		\edef\@yoffc{\number\@result\space\space}

	\in@atbdc{\@xoff}{\@xscale}{100} \edef\@xoff{\number\@result\space\space}
	\in@atbdc{\@xoffa}{\@xscalea}{100} \edef\@xoffa{\number\@result\space\space}
	\in@atbdc{\@xoffb}{\@xscaleb}{100} \edef\@xoffb{\number\@result\space\space}
	\in@atbdc{\@xoffc}{\@xscalec}{100} \edef\@xoffc{\number\@result\space\space}
	\in@atbdc{\@yoff}{\@yscale}{100} \edef\@yoff{\number\@result\space\space}
	\in@atbdc{\@yoffa}{\@yscalea}{100} \edef\@yoffa{\number\@result\space\space}
	\in@atbdc{\@yoffb}{\@yscaleb}{100} \edef\@yoffb{\number\@result\space\space}
	\in@atbdc{\@yoffc}{\@yscalec}{100} \edef\@yoffc{\number\@result\space\space}
%
%   Give warning when the figures are too wide.
%
\dimen0=\@hsizee pt	
\ifdim \dimen0 >\hsize
	\typeout{----- FourFigures warning: ps figures are too wide ! }
\fi
%
	\vskip 10pt \nobreak
	\hbox to \hsize{
		\hss
		\dimen0= \@hsizee pt
		\hbox to \dimen0 {
			\dimen0= \@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfile }
					\special{psfile=\@p@sfile
						hoffset = \@xoff
						voffset = \@yoff
						hscale=\@xscale 
						vscale=\@yscale}
					 }
					\hss
			\dimen0= \@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfilea }
					\special{psfile=\@p@sfilea
						hoffset = \@xoffa
						voffset = \@yoffa
						hscale=\@xscalea 
						vscale=\@yscalea}
					 }
					\hss
			\dimen0=\@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfileb }
					\special{psfile=\@p@sfileb
						hoffset = \@xoffb
						voffset = \@yoffb
						hscale=\@xscaleb 
						vscale=\@yscaleb}
					}
					\hss
			\dimen0=\@maxh pt
			\vbox to \dimen0{
					\vss
%	\typeout{----- FIG: including \@p@sfilec }
					\special{psfile=\@p@sfilec
						hoffset = \@xoffc
						voffset = \@yoffc
						hscale=\@xscalec
						vscale=\@yscalec}
					}
					\hss
				}
			\hss
		}
	\vskip 6pt \nobreak
	\centerline{#5}
	\vskip 4pt
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=12\relax
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

